A randomized algorithm for simultaneously diagonalizing symmetric matrices by congruence

A family of symmetric matrices $A_1,\ldots, A_d$ is SDC (simultaneous diagonalization by congruence, also called non-orthogonal joint diagonalization) if there is an invertible matrix $X$ such that every $X^T A_k X$ is diagonal. In this work, a novel randomized SDC (RSDC) algorithm is proposed that reduces SDC to a generalized eigenvalue problem by considering two (random) linear combinations of the family. We establish exact recovery: RSDC achieves diagonalization with probability $1$ if the family is exactly SDC. Under a mild regularity assumption, robust recovery is also established: Given a family that is $\epsilon$-close to SDC then RSDC diagonalizes, with high probability, the family up to an error of norm $\mathcal{O}(\epsilon)$. Under a positive definiteness assumption, which often holds in applications, stronger results are established, including a bound on the condition number of the transformation matrix. For practical use, we suggest to combine RSDC with an optimization algorithm. The performance of the resulting method is verified for synthetic data, image separation and EEG analysis tasks. It turns out that our newly developed method outperforms existing optimization-based methods in terms of efficiency while achieving a comparable level of accuracy.

==> RFFDIAG.tex <==
\section{Refinement using FFDIAG}

Unlike in the orthogonal JD case, for SDC, it is not obvious to come up with a deflation-based algorithm like Algorithm $2$ in \cite{he2022randomized} for refinement because the columns of $\tilde X$ is not orthogonal. However, according to Theorem \ref{thm:pd_prob_bound} and Theorem \ref{thm:npd_prob_bound}, with high probability, the output of Algorithm \ref{alg:RSDC} will be a good initial guess for optimization algorithms.  The particular optimization algorithm considered in this paper is FFDIAG\cite{Ziehe03}.


Since the output of Algorithm \ref{alg:RSDC}, RSDC, will be relatively accurate with high probability, we expect that FFDIAG will converge within few iterations with setting the initial point as the output of RSDC with only $1$ trial. The Randomized FFDIAG is summarized in Algorithm \ref{alg:RRSDC}.   In practice,  we consider $d=10$ SDC matrices of size $100 \times 100$, it is observed as in Table \ref{table:rffdiag_iters} that the RSDC drastically reduced the number of iterations of FFDIAG. More numerical experiments on accuracy and running time will be covered in Section \ref{sec:numerical_experiments}.


\begin{algorithm}[H]
\caption{\textbf{R}andomized \textbf{FFDIAG} (RFFDIAG)}
\label{alg:RRSDC}
\textbf{Input:} \text{$\tilde{\Acal} =\{\tilde{A}_k \in \reals^{n \times n}\}_{k=1}^{d}$, number of iterations $N$.}\\
 \textbf{Output:} \text{The simultaneous diagonalizer $\tilde{X}$.}
\begin{algorithmic}[1]
\STATE $\tilde X_0 = \text{RSDC}(\tilde {\mathcal{A}}, 1)$ with suitable distributions of $\mu, \theta$
\STATE $\tilde X = \text{FFDIAG}(\tilde X_0,  \tilde{\Acal})$ 
\RETURN $\tilde X$

\end{algorithmic}
\end{algorithm}


\begin{table}[!hbt!]
    \begin{center}
    \caption{Number of iterations comparison FFDIAG vs RFFDIAG}
    \label{table:rffdiag_iters}
    \begin{tabular}{||c | c | |}
    \hline
    Algorithm & \# of iterations\\
    \hline
    FFDIAG & $\num{47}$\\
    \hline
    RFFDIAG & $\num{1}$\\
    \hline
    \end{tabular}
    \end{center}
\end{table}


==> RFFDIAG_RRCG.tex <==

\section{Iterative refinement}\label{sec:iterative_refinement}
In contrast to the orthogonal JD case, for SDC, coming up with a deflation-based algorithm akin to Algorithm $2$ in \cite{he2022randomized} for refinement is not straight forward, because the columns of $\tilde X$ is not orthogonal. However, according to Theorem \ref{thm:npd_prob_bound} and Theorem \ref{thm:pd_prob_bound}, with high probability, the output of Algorithm \ref{alg:RSDC} will be a good starting point for optimization algorithms. The particular optimization algorithms considered in this paper are Riemannian Conjugate Gradient(RCG) and FFDIAG~\cite{Ziehe03}.

\subsection{Randomized RCG}
Let us give a brief introduction to Riemannian optimization. We refer the readers again to the textbooks\cite{AbsMahSep2008,boumal2023intromanifolds} for a complete overview.  Riemannian optimization is concerned with 
\[\min_{x \in \mathcal{M}} f(x)\]
where $f$ is a smooth objective function defined on the Riemannian manifold $\mathcal{M}$. In our setting, we use the objective function \eqref{eq:off_diagonal_loss} and the manifold of interest $\mathcal{M}$ is the oblique manifold $\OB(n,n)$ \eqref{eq:oblique_manifold}. Similar to Euclidean Conjugate Gradient (CG),  Riemannian Conjugate Gradient (RCG) improves the descent directions by combining the current gradient and the directions from previous updates. However, to ensure each updated point still stays on the manifold, we need retractions~\cite[Definition 3.47]{boumal2023intromanifolds}
\[R: T\mathcal{M} \to \mathcal{M}: (x,v) \mapsto R_x(v),\]which generalizes the concept of straight lines in the Euclidean spaces. Unlike in the Euclidean setting, for Riemannian optimization, a vector transport\cite[Definition 8.1.1]{AbsMahSep2008}
 \[\mathcal{T}_u: \mathcal{T}_x \mathcal{M} \to \mathcal{T}_{R_x(u)} \mathcal{M}, u \in \mathcal{T}_x\mathcal{M}   \]
bringing vectors in $ \mathcal{T}_x\mathcal{M}$ to $\mathcal{T}_{R_u(x)} \mathcal{M}$
is needed to bring update directions at different iterations to the same tangent space to generate the new search direction. The RCG algorithm is summarized in Algorithm \ref{alg:RCG}. We use the existing implementation available in \textsc{Pymanopt} package\cite{pymanopt} with the backtracking line-search algorithm \cite[Algorithm 4.2]{boumal2023intromanifolds} and Hestenes-Stiefel update rule \cite{HestenesStiefel52} throughout this paper\footnote{The \textsc{Pymanopt} package is documented at \url{https://pymanopt.org/}}.



\begin{algorithm}[H]
\caption{\textbf{R}iemannian \textbf{C}onjugate \textbf{G}radient (RCG)}
\textbf{Input:} \text{$X_0 \in \mathcal{M}$, $f: \mathcal{M} \to \reals$, $k_{\max} \in \mathbb{N}^+$}
\begin{algorithmic}[1]
\label{alg:RCG}
\STATE $k = 0$
\STATE $V_0 = -\grad f(X_k)$
\WHILE{$k < k_{\max}$ \AND $\|\grad f(X_k)\|_{X_k} > \epsilon_{\text{tol}}$}
    \STATE Choose the step size $\alpha_k$ by the backtracking line-search algorithm 
    \STATE $X_{k+1} = R_{X_k}(\alpha_kV_k)$
    \STATE Compute $\beta_{k+1}$ by Hestenes-Stiefel update rule.
    \STATE $V_{k+1} = - \grad f(X_{k+1}) + \beta_{k+1}\mathcal{T}_{\alpha_kV_k}(\grad f(X_k))$
    \STATE $k = k + 1$
\ENDWHILE
\RETURN $X_k$
\end{algorithmic}
\end{algorithm}

The Riemannian optimization based RSDC is summarized in Algorithm \ref{alg:RRSDC}. If we run RCG directly without the randomized initial point, the number of iterations is far from comparable with RRSDC. In practice, the number of iterations $N$ can be set to a small number such as $10$. See more about the number of iterations in Section \ref{sec:numerical_experiments}. 

\begin{algorithm}[H]
\caption{\textbf{R}iemannian optimization based \textbf{RSDC} (RRSDC)}
\label{alg:RRSDC}
\textbf{Input:} \text{$\tilde{\Acal} =\{\tilde{A}_k \in \reals^{n \times n}\}_{k=1}^{d}$, number of trials $L$, number of iterations $N$.}\\
 \textbf{Output:} \text{The simultaneous diagonalizer $\tilde{X}$.}
\begin{algorithmic}[1]
\STATE $\tilde X_0 = \text{RSDC}(\tilde {\mathcal{A}}, L)$ with suitable distributions of $\mu, \theta$
\STATE $\tilde X = \text{RCG}(\tilde X_0,  \mathcal{L},  N)$ \textit {$\mathcal{L}$ is described in \eqref{eq:off_diagonal_loss}}
\RETURN $\tilde X$

\end{algorithmic}
\end{algorithm}

\subsection{Randomized FFDIAG}

FFDIAG is a quasi-Newton's method to minimize the loss \eqref{eq:off_diagonal_loss} by multiplication update of the diagonalizer $\tilde X$, i.e, $\tilde X_{k+1} = (I+W)\tilde X_k$ for some carefully chosen $W$. For more details on FFDIAG, we refer the reader to \cite[Algorithm 1]{Ziehe03}. In \cite{Ziehe03}, it is also mentioned that a smarter way of initializing instead of only using $I_n$ should be investigated, and our RSDC is a perfect smart initial guess.

The Randomized FFDIAG is summarized in Algorithm \ref{alg:RRSDC}. In practice, we consider $d=10$ SDC matrices of size $100 \times 100$, it is observed as in Table \ref{table:rffdiag_iters} that the RSDC drastically reduced the number of iterations of FFDIAG. And like RRSDC, the number of iterations of FFDIAG can also be set to only $10$. More numerical experiments on accuracy and running time will be covered in Section \ref{sec:numerical_experiments}.


\begin{algorithm}[H]
\caption{\textbf{R}andomized \textbf{FFDIAG} (RFFDIAG)}
\label{alg:RFFDIAG}
\textbf{Input:} \text{$\tilde{\Acal} =\{\tilde{A}_k \in \reals^{n \times n}\}_{k=1}^{d}$, number of iterations $N$.}\\
 \textbf{Output:} \text{The simultaneous diagonalizer $\tilde{X}$.}
\begin{algorithmic}[1]
\STATE $\tilde X_0 = \text{RSDC}(\tilde {\mathcal{A}}, 1)$ with suitable distributions of $\mu, \theta$
\STATE $\tilde X = \text{FFDIAG}(\tilde X_0,  \tilde{\Acal})$ 
\RETURN $\tilde X$

\end{algorithmic}
\end{algorithm}


\begin{table}[!hbt!]
    \begin{center}
    \caption{Number of iterations comparison FFDIAG vs RFFDIAG}
    \label{table:rffdiag_iters}
    \begin{tabular}{||c | c | |}
    \hline
    Algorithm & \# of iterations\\
    \hline
    FFDIAG & $\num{47}$\\
    \hline
    RFFDIAG & $\num{1}$\\
    \hline
    \end{tabular}
    \end{center}
\end{table}

It is worth mentioning before diving into the numerical experiments that RFFDIAG is better than RRSDC in terms of both accuracy and efficiency.

==> RSDC_manopt.tex <==
\section{Refinement using Riemannian CG}

Unlike in the orthogonal JD case, for SDC, it is not obvious to come up with a deflation-based algorithm like Algorithm $2$ in \cite{he2022randomized} for refinement because the columns of $\tilde X$ is not orthogonal. However, according to Theorem \ref{thm:pd_prob_bound} and Theorem \ref{thm:npd_prob_bound}, with high probability, the output of Algorithm \ref{alg:RSDC} will be a good initial guess for optimization algorithms.  The particular optimization algorithm considered in this paper is Riemannian Conjugate Gradient(RCG).

Let us give a brief introduction to Riemannian optimization. We refer the readers again to the textbooks\cite{AbsMahSep2008,boumal2023intromanifolds} for a complete overview.  Riemannian optimization is concerned with 
\[\min_{x \in \mathcal{M}} f(x)\]
where $f$ is a smooth objective function defined on the Riemannian manifold $\mathcal{M}$. In our setting, we use the objective function \eqref{eq:off_diagonal_loss} and the manifold of interest $\mathcal{M}$ is the oblique manifold $\OB(n,n)$ \eqref{eq:oblique_manifold}. Similar to Euclidean Conjugate Gradient (CG),  Riemannian Conjugate Gradient (RCG) improves the descent directions by combining the current gradient and the directions from previous updates. However, to ensure each updated point still stays on the manifold, we need retractions \cite[Definition 3.47]{boumal2023intromanifolds}
\[R: T\mathcal{M} \to \mathcal{M}: (x,v) \mapsto R_x(v),\]which generalizes the concept of straight lines in the Euclidean spaces. Unlike in the Euclidean setting, for Riemannian optimization, a vector transport\cite[Definition 8.1.1]{AbsMahSep2008}
 \[\mathcal{T}_u: \mathcal{T}_x \mathcal{M} \to \mathcal{T}_{R_x(u)} \mathcal{M}, u \in \mathcal{T}_x\mathcal{M}   \]
bringing vectors in $ \mathcal{T}_x\mathcal{M}$ to $\mathcal{T}_{R_u(x)} \mathcal{M}$
is needed to bring update directions at different iterations to the same tangent space to generate the new search direction. The RCG algorithm is summarized in Algorithm \ref{alg:RCG}. We use the existing implementation available in \textsc{Pymanopt} package\cite{pymanopt} with the backtracking line-search algorithm \cite[Algorithm 4.2]{boumal2023intromanifolds} and Hestenes-Stiefel update rule \cite{HestenesStiefel52} throughout this paper\footnote{The \textsc{Pymanopt} package is documented at \url{https://pymanopt.org/}}.



\begin{algorithm}[H]
\caption{\textbf{R}iemannian \textbf{C}onjugate \textbf{G}radient (RCG)}
\textbf{Input:} \text{$X_0 \in \mathcal{M}$, $f: \mathcal{M} \to \reals$, $k_{\max} \in \mathbb{N}^+$}
\begin{algorithmic}[1]
\label{alg:RCG}
\STATE $k = 0$
\STATE $V_0 = -\grad f(X_k)$
\WHILE{$k < k_{\max}$ \AND $\|\grad f(X_k)\|_{X_k} > \epsilon_{\text{tol}}$}
    \STATE Choose the step size $\alpha_k$ by the backtracking line-search algorithm 
    \STATE $X_{k+1} = R_{X_k}(\alpha_kV_k)$
    \STATE Compute $\beta_{k+1}$ by Hestenes-Stiefel update rule.
    \STATE $V_{k+1} = - \grad f(X_{k+1}) + \beta_{k+1}\mathcal{T}_{\alpha_kV_k}(\grad f(X_k))$
    \STATE $k = k + 1$
\ENDWHILE
\RETURN $X_k$
\end{algorithmic}
\end{algorithm}

Since the output of Algorithm \ref{alg:RSDC}, RSDC, will be relatively accurate with high probability, we only need to consider running few iterations of RCG for refinement. In practice, the number of iterations $N$ can be set to a small number such as $10$. See more about the number of iterations in Section \ref{sec:numerical_experiments}. The Riemannian optimization based RSDC is summarized in Algorithm \ref{alg:RRSDC}. 

\begin{algorithm}[H]
\caption{\textbf{R}iemannian optimization based \textbf{RSDC} (RRSDC)}
\label{alg:RRSDC}
\textbf{Input:} \text{$\tilde{\Acal} =\{\tilde{A}_k \in \reals^{n \times n}\}_{k=1}^{d}$, number of trials $L$, number of iterations $N$.}\\
 \textbf{Output:} \text{The simultaneous diagonalizer $\tilde{X}$.}
\begin{algorithmic}[1]
\STATE $\tilde X_0 = \text{RSDC}(\tilde {\mathcal{A}}, L)$ with suitable distributions of $\mu, \theta$
\STATE $\tilde X = \text{RCG}(\tilde X_0,  \mathcal{L},  N)$ \textit {$\mathcal{L}$ is described in \eqref{eq:off_diagonal_loss}}
\RETURN $\tilde X$

\end{algorithmic}
\end{algorithm}



==> backup_theorem_14.tex <==
\begin{theorem}[Main theorem for regular families]
\label{thm:npd_prob_bound_new}
Under the setting of Theorem~\ref{thm:structural_bound}, assume that $\theta, \mu$ are independent Gaussian random vectors. \revise{Let} $\tilde X$ 
be any invertible matrix such that $\tilde X^T \tilde A(\mu) \tilde X$ and $\tilde X^T \tilde A(\theta) \tilde X$ are diagonal. Then, for any $R > 0$, it holds that
    \begin{align*}
\Prob\Big(\frac{1}{\|\tilde X\|_2^2}\Big(\sum_{k=1}^{d}\fnormbig{\offdiag(\tilde{X}^T\tilde{A}_k\tilde{X})}^2\Big)^{1/2} &\leq (R^2 + 1) \epsilon  + \Ocal(\epsilon^2)\Big) \\ &\geq 1 - \frac{\sqrt{5}}{\sqrt{2\pi}}\frac{m^{3/2} d^{3/4}}{R}.
\end{align*}
\end{theorem}
\begin{proof} 
Since the invertibility of $A(\theta)$ holds almost surely, one can apply
Theorem~\ref{thm:structural_bound}, which yields the following bound:
\begin{align}\label{eq:nonpd_structural_bound}
&\frac{1}{\|\tilde X\|_2^2} \Big(\sum_{k=1}^{d}\big\|\offdiag(\tilde X^T \tilde A_k \tilde X) \big\|_F^2 \Big)^{1/2} \nonumber \\
\leq& \sqrt{d} \big( D_{\max} \|E(\mu)\|_F + ( \lambda^\mu_{\max} D_{\max} + \lambda_{\max})  \|E(\theta)\|_F\big)\epsilon + \epsilon + \mathcal O(\epsilon^2).
\end{align}
When $m = 1$, $D_{\text{max}} = 0$, applying bound of Lemma \ref{lemma:control_theta} to the above bound yields
\[\frac{1}{\|\tilde X\|_2^2} \Big(\sum_{k=1}^{d}\big\|\offdiag(\tilde X^T \tilde A_k \tilde X) \big\|_F^2 \Big)^{1/2} \leq \sqrt{d}C\epsilon + \epsilon + \mathcal O(\epsilon^2)\]
with probability $1- \sqrt{2d/\pi} /C$.  Since $d\geq 2$, this bound becomes negative when $C< 1$ and, in turn, the result of the theorem trivially holds. We may therefore assume $C\geq 1$ in the following.  The substitution $C = R^2/\sqrt{d} $ together with the condition $C\geq1$ give us
\[\frac{1}{\|\tilde X\|_2^2} \Big(\sum_{k=1}^{d}\big\|\offdiag(\tilde X^T \tilde A_k \tilde X) \big\|_F^2 \Big)^{1/2} \leq R^2\epsilon + \epsilon + \mathcal O(\epsilon^2)\]
with probability $1- \sqrt{2/\pi}d /R^2 \geq 1 - \sqrt{2/\pi}d^{3/4} / R \leq 1 - \sqrt{5/2\pi}d^{3/4} / R$.

When $m\geq 2$, given $R > 0$, we set $R_0 =((5/2)\sqrt{d})^{1/2}R/\sqrt{2m}$. By the union bound, the bounds of Lemma~\ref{lemma:failure_prob} for $R_0>0$ and Lemma~\ref{lemma:control_theta} for $C = 2R_0/m$ hold, with probability at least
\begin{equation} \label{eq:success_new}
 1-\sqrt{\frac{d}{2\pi}}\frac{m(m-1)}{R_0} - \sqrt{\frac{2d}{\pi}}\frac{m}{C} \leq 1-\sqrt{\frac{d}{2\pi}}2\frac{m^2}{R_0} = 1-.
\end{equation}
Since $d\geq 2$, this bound becomes negative when $R_0 < m^2$ and, in turn, the result of the theorem trivially holds. We may therefore assume $R_0 \geq m^2$ in the following.
Applying the bound  \eqref{eq:success_new} to \eqref{eq:nonpd_structural_bound} yields 
\begin{align*}
    \frac{1}{\|\tilde X\|_2^2} \Big(\sum_{k=1}^{d}\big\|\offdiag(\tilde X^T \tilde A_k \tilde X) \big\|_F^2 \Big)^{1/2} &\leq \sqrt{d}\big( R_0 + CR_0 + C\big)\epsilon + \epsilon + \mathcal O(\epsilon^2)\\
    &= \sqrt{d}(m/R_0 + 1 + 1/R_0)R_0^2/m\epsilon +  \epsilon + \mathcal O(\epsilon^2)\\
    &\leq \big((5/2)\sqrt{d}R_0^2/m\big)\epsilon  +  \epsilon + \mathcal O(\epsilon^2)
\end{align*}
where we used $R_0\ge m \geq 2$ in the last inequality. Performing the substitution
$R\gets ( m R^2 / 5 \sqrt{d})^{1/2}$ completes the proof.
\end{proof}

\begin{theorem}[Main theorem for regular families]
\label{thm:npd_prob_bound}
Under the setting of Theorem~\ref{thm:structural_bound}, assume that $\theta, \mu$ are independent Gaussian random vectors. \revise{Let} $\tilde X$ 
be any invertible matrix such that $\tilde X^T \tilde A(\mu) \tilde X$ and $\tilde X^T \tilde A(\theta) \tilde X$ are diagonal. \revise{Then, for any $R > 0$, it holds that}
    \begin{align*}
\Prob\Bigg(\frac{1}{\|\tilde X\|_2^2}\Big(\sum_{k=1}^{d}\fnormbig{\offdiag(\tilde{X}^T\tilde{A}_k\tilde{X})}^2\Big)^{1/2} &\leq (R^2 + 1) \epsilon  + \Ocal(\epsilon^2)\Bigg) \\ &\geq 1 - \revise{\sqrt{2}} \frac{m^{3/2} d^{3/4}}{R}.
\end{align*}
\end{theorem}
\begin{proof}
\revise{Given $R>0$, we set $R_0 = R \sqrt{m} / \sqrt{4\pi \sqrt{d}} > 0$.} By the union bound, the bounds of Lemma~\ref{lemma:failure_prob} \revise{for $R_0$} and \revise{ Lemma~\ref{lemma:control_theta} for $C = 2 \revise{R_0} / m$} hold, with probability at least
\begin{equation} \label{eq:success}
 1-\sqrt{\frac{d}{2\pi}}\frac{m(m-1)}{\revise{R_0}} - \sqrt{\frac{2d}{\pi}}\frac{m}{C} \ge 
 1-\sqrt{\frac{\revise{2d}}{\pi}}\frac{m^2}{\revise{R_0}} \revise{ = 1 - \sqrt{2} \frac{m^{3/2} d^{3/4}}{R}},
\end{equation}
\revise{Because $d \ge 2$, this bound becomes negative when $R_0 < m/\sqrt{\pi}$ and, in turn, the result of the theorem trivially holds. We may therefore assume $R_0 \ge m/\sqrt{\pi}$ in the following.}
\revise{Since} the invertibility of $A(\theta)$ holds \revise{almost surely}, \revise{one can apply}
Theorem~\ref{thm:structural_bound}, which yields the following bound:
\textcolor{blue}{\begin{align*}
&\frac{1}{\|\tilde X\|_2^2} \Big(\sum_{k=1}^{d}\big\|\offdiag(\tilde X^T \tilde A_k \tilde X) \big\|_F^2 \Big)^{1/2} \\
\leq& \sqrt{d} \big( D_{\max} \|E(\mu)\|_F + ( \lambda^\mu_{\max} D_{\max} + \lambda_{\max})  \|E(\theta)\|_F\big)\epsilon + \epsilon + \mathcal O(\epsilon^2) \\
\le& \sqrt{d} ( \revise{R_0} + C \revise{R_0} + C)\epsilon + \epsilon + \mathcal O(\epsilon^2) \\
=& \sqrt{d} \big( m / \revise{R_0} + 2  + 2 / R_0\big)\revise{R_0}^2/m\cdot \epsilon + \epsilon + \mathcal O(\epsilon^2) \\
\le & \sqrt{d} ( 3 \sqrt{\pi} + 2 ) R^2_0 /m \cdot \epsilon + \epsilon + \mathcal O(\epsilon^2)  \\
\le & ( 4 \pi  \sqrt{d}  \revise{R_0}^2 /m )\epsilon + \epsilon + \mathcal O(\epsilon^2) = ( R^2 + 1 ) \epsilon + \mathcal O(\epsilon^2).
\end{align*}}%
\revise{Here, the second inequality follows from the bounds of Lemmas~\ref{lemma:failure_prob} and~\ref{lemma:control_theta}. The third inequality
uses that $R_0 \ge m/\sqrt{\pi}$ implies $(m+2) /R_0 \le  3 \sqrt{\pi}$.}
\end{proof}

==> implementation_detail_backup.tex <==
\section{Implementation details}
\label{sec:implementation_details}
In this section, we discuss how we solve Line 3 in Algorithm \ref{alg:RSDC} and how can we boost the success probability by multiple trials. The detailed implementation of Algorithm \ref{alg:RSDC} is summarized in Algorithm \ref{alg:detailed_RSDC}.

In Line 3 of Algorithm \ref{alg:RSDC}, we need to SDC two random linear combinations $\tilde A(\theta), \tilde A(\mu)$ if we input the nearly SDC family $\tilde \Acal = \{VD_kV^T+E_k\}$ into the Algorithm \ref{alg:RSDC}. As we already discussed in Example \ref{example:nonsdc} and \ref{example:small_perturbtaion_nonsdc}, $(\tilde A(\theta), \tilde A(\mu))$ might not be SDC in general. We assume $\tilde \Acal$ is a regular diagonalizable family. As indicated in the proof of Proposition \ref{prop:diag_imply_sdc}, if there is no multiplicity in the generalized eigenvalues of the pair, we can SDC this pair via a generalized eigenvalue problem 
\[\tilde A(\theta) \tilde X \Theta =  \tilde A(\mu) \tilde X \Lambda.\]
 However, when there is multiplicity in the generalized eigenvalues of $(\tilde A(\mu), \tilde A(\theta))$, $\tilde X^T \tilde A(\mu) \tilde X$ and $\tilde X^T \tilde A(\theta) \tilde X$ might not be diagonal. Fortunately, as indicated in the proof of Proposition \ref{prop:diag_imply_sdc}, $\tilde X^T \tilde A(\mu) \tilde X$ and $\tilde X^T \tilde A(\theta) \tilde X$ commute and thanks to the recent development of orthogonal joint diagonalization(JD) for commuting pairs \cite{he2022randomized,Sutton23}, we can always SDC  $(\tilde A(\mu), \tilde A(\theta))$ by solving the generalized eigenvalue problem followed by an orthogonal JD on $(\tilde X^T\tilde A(\mu)\tilde X, \tilde X \tilde A(\theta) \tilde X)$ efficiently. In practice, we observe that the orthogonal joint diagonalization step is not necessary. Thus, we only apply LAPACK's~\cite{LAPACK} QZ algorithm~\cite{kressner05,matrixcomputation} to obtain $\tilde X$ and consider the orthogonal joint diagonalization step optional.

 Furthermore, we can boost the success probability of Algorithm \ref{alg:RSDC} by picking the best candidates among multiple trials in terms of the measure \eqref{eq:off_diagonal_loss}. Nevertheless, \eqref{eq:off_diagonal_loss} is not invariant of column scaling, in order to compare the quality of different trials, it is necessary to normalize the columns of each output to have norm $1$. The complete algorithm is summarized in Algorithm \ref{alg:detailed_RSDC}.
\begin{algorithm}[H]
    \caption{\textbf{R}andomized \textbf{S}imultaneous \textbf{D}iagonalization via \textbf{C}ongruence (RSDC)}
    \textbf{Input:} \text{A nearly SDC family $\tilde{\Acal} =\{\tilde{A}_k \in \reals^{n \times n}\}_{k=1}^{d}$, number of trials $L$.}\\
     \textbf{Output:} \text{The simultaneous diagonalizer $\tilde{X}$.}
    \begin{algorithmic}[1]
    \label{alg:detailed_RSDC}
    \FOR{$i=1$ to $L$}
        \STATE Draw $\mu^{(i)}, \theta^{(i)}$ from specific distribution.
        \STATE Compute $\tilde{A}(\mu^{(i)}) = \mu_1^{(i)} \tilde A_1 + \cdots + \theta_d^{(i)} \tilde A_d$, $\tilde{A}(\theta^{(i)}) = \theta_1^{(i)} \tilde A_1 + \cdots + \theta_d^{(i)} \tilde A_d$.
        \STATE $\tilde X_i = \text{QZ}(\tilde A(\mu), \tilde A(\theta))$.
        \STATE [optional] $Q_i = \text{JD}(\tilde X_i^T \tilde A(\mu) \tilde X_i,\tilde X_i^T \tilde A(\theta) \tilde X_i )$, $\tilde X_i \leftarrow \tilde X_i Q_i$.
        \STATE Normalize $\tilde X_i$ so that its has column norms equal to $1$.
    \ENDFOR
    \STATE Let $i^* = \argmin_{i}\Big\{ \sum_{k = 1}^{d}\fnormbig{\offdiag(\tilde{X}_i^T \tilde{A}_k \tilde{X}_i)}^2\Big\}$.
    \RETURN $\tilde{X}_{i^*}$
    \end{algorithmic}
    \end{algorithm}

==> numerical_experiments_backup.tex <==


\section{Numerical experiments}

Throughout the experiments in this section, we only consider $3$ trails to boost the success probability of RSDC and RRSDC. And the number of maximum iterations of RRSDC and RFFDIAG are both set to $10$. Note that the accuracy can be further improved by both more trials of the RSDC and more iterations of RCG and FFDIAG, but at the cost of efficiency. The code is available at:  \\
All the experiments were implemented using Python 3.8 and were executed on a Dell XPS 13 2-In-1 with an Intel Core i7-1165G7 CPU and 16GB of RAM. The running times reported throughout this paper are consistently in milliseconds.

\label{sec:numerical_experiments}
\subsection{Synthetic data}

The nearly SDC families $\tilde \Acal = \{\tilde A_k = VD_kV^T + E_k \in \reals^{n \times n}\}_{k=1}^{d}$ are generated with different values of $n,d$. $V$ is first picked as a Gaussian random matrix where each entry follows i.i.d standard Gaussian distribution. Then $V$ is normalized to have column norm $1$. Entries of $D_k$ follow i.i.d distribution $0.01 + |\Normal{0}{1}|$ as competing methods QNDIAG and PHAM require positive definiteness (Our algorithms do not require). 
We consider three different sizes $(d,n) = (10,10), (100,10), (10,100)$ and three different noise levels $\epsilon = (\sum_{k=1}^{d}\fnorm{E_k}^2)^{1/2}$, $\epsilon_1 = 0$, $\epsilon_2 = 10 ^{-6}$ and $\epsilon_3 = 10^{-3}$. The setting $(10,10)$ acts as a sanity check, while $(100,10)$ and $(10,100)$ settings imitate the situation where we get a large number of SDC matrices and a family of SDC matrices with large sizes respectively. As QNDIAG and PHAM assume positive definite matrices , we enforce positive definiteness by repeatedly generating the errors $E_k,k=1,\ldots,d$ until all the matrices in the family  $\tilde \Acal$  are positive definite. We normalize the columns of the output matrices from all the algorithms to have norm $1$ so that the error is comparable among different algorithms. The results are shown in the Table \ref{table:RSDC_10_10} to \ref{table:RSDC_10_100}.
%\input{table_error_runtime_rsdc}
\input{table_error_runtime_rffdiag.tex}

We also test the algorithms on relatively ill-conditioned matrices. For this scenario, we set $\epsilon = 0$ and $d = 20, n = 30$. $V$ is generated in the same way as above, while entries of $D_k$ is random permutations of the vector \[\begin{bmatrix} 10^{0} & 10^{8/(n-1)} &  10^{16/(n-1)} & \ldots &  10^{8}\end{bmatrix}^T.\]  The result is shown in Table \ref{table:ill_conditioned_rsdc}. It can be observed that algorithms PHAM and QNDIAG, which are based on the loss \eqref{eq:pham_loss}, are not robust when the matrices are not well-conditioned.
\input{table_error_rumtime_rffdiag_ill_conditioned.tex}

From all the above experiments on synthetic data, we can safely conclude that RFFDIAG reaches the best performance in both accuracy and efficiency. Next we move on to test RFFDIAG on some real-world examples in BSS.

\subsection{Application: Blind Source Separation}
In Blind Source Separartion (BSS), for $n$ source signals $s_j(t)$, $j=1,\ldots,n$, the observed $n$ signals $x_j(t)$, $j=1,\ldots,n$ are assumed to be linear mixture of the source signals. I.e., 
\[x_i(t) = \sum_{j = 1}^{n} A_{ij}s_j(t)\]
where $A \in \reals^{n \times n}$ is a non-singular matrix. The task of BSS is to estimate a matrix $B$ only from the observed signals such that the unmixed signals $(Bx)_j(t)$ is a scalar multiple of some source signal $s_j(t)$. See, e.g, \cite{BSSsurvey} for an overview on BSS. The unmixing matrix $B$ can be estimated by performing SDC on second-order statistics, e.g., time-lagged covariance matrices \cite{Belouchrani1997}, Fourier cospectra~\cite{BARTHELEMY2017371}, or even covariance matrices of different signal segments~\cite{Pham2001IEEE},  of the observed signals $x_i(t)$. The experiments conducted in the following two subsections are two real-world examples of BSS.


\subsection{Real data: image separation}
Following Example 1 in \cite{Pfister2019}, we conduct a similar image separation experiment. The source signals in this example are vectorized images of landscapes. We mixed the same $4$ photos of landscapes as in \cite{Pfister2019} with a random Gaussian mixing matrix $A \in \reals^{4 \times 4}$, i.e, entries of $A \sim \Normal{0}{1}$.

We then compute the covariance matrices of different signal segments of the observed mixed signals, which results in $1350$ $4 \times 4$ matrices to be jointly diagonalized. We apply our RSDC and RFFDIAG on this family of nearly SDC matrices, and compare with the default SDC solver UWEDGE \cite{uwedge} in this scenario. The separation result is shown in Figure \ref{fig:image_separartion}. The original landscapes are displayed in the first rows, and the observed mixtures are in the second rows, followed by separation results from different SDC algorithms. The running time, averaged over 100 runs, of each algorithm is reported in Table \ref{table:image_separartion_runningtime}.

From the result, it can be observed by eye that although RSDC achieves a significant improvement in efficiency, $20$ times faster than the default UWEDGE, the landscape reconstructions are noisy. UWEDGE and RFFDIAG both lead to almost perfect reconstruction of the original images, while RFFDIAG runs significantly faster than the default UWEDGE.
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{picture_example_ffdiag.pdf}
    \caption{Images of the image separartion example, the first row show the original images, the second row show the mixed images, and the last 3 rows show the unmixed images from different SDC algorithms RSDC, RFFDIAG, and UWEDGE. }
    \label{fig:image_separartion}
\end{figure}
\input{table_image_separation_runningtime_rffdiag}
\subsection{Real data: electroencephalographic recordings}
We test our randomized SDC algorithms on real electroencephalographic (EEG) recordings. In Human EEG, it is known that \cite[Chapter 8.2]{Congedo2014} the signals observed in the different electrodes on the scalp are approximately linear mixture of the source signals in the brain. It is proposed in \cite{BARTHELEMY2017371} that the eye-blinking noise signal can be separated by performing SDC on the Fourier cospectra
of the EEG recording. We follow the implementation in \cite{pyriemann}\footnote{\href{https://pyriemann.readthedocs.io/}{https://pyriemann.readthedocs.io/}}, where they use SDC solver introduced in \cite{Pham2001} as default. In this experiment, we have $d=33$ matrices of size $17\times 17$ to be SDC. Note that in some other BSSs task in EEG, the number of matrices and the size of the matrices can both be much larger\cite{}, where efficiency could be a large concern. The power spectrum and the topograhpic map of the estimated blink source signal is shown in Figure \ref{fig:pham_blink_source}. We can see that, from the topographic map of the source signal on the scalp, the source signal is indeed concentrated among eyes, which confirms that this signal corresponds to eye-blink. 

We applied our RSDC and RFFDIAG to the same data, and the results are shown in Figure \ref{fig:Manrsdc_blink_source} and Figure \ref{fig:rsdc_blink_source} respectively. From the figures we can see that both the algorithms identify the blink signals successfully and the their power spectrum are also close to the one estimated by the default solver. However, compared RSDC with RFFDIAG and Pham, we can observe from the topograhic map that the result of RSDC is a bit more noisy.

Next, we compare the running time of different SDC algorithms involved in this BSS task.
All the running times are again averaged over $100$ runs. See Table \ref{table:eeg_runningtime}. It can be clearly seen that RSDC and RFFDIAG run significantly faster than the default Pham algorithm on this real EEG data while still achieve a satisfactory level of accuracy.
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{Pham_blink_source.jpg}
    \caption{Power spectrum and topograhic map of the blink source by Pham}
    \label{fig:pham_blink_source}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{rsdc_blink_source.jpg}
    \caption{Power spectrum and topograhic map of the blink source by RSDC}
    \label{fig:rsdc_blink_source}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{FFDIAG_blink_source.jpg}
    \caption{Power spectrum and topograhic map of the blink source by RFFDIAG}
    \label{fig:Manrsdc_blink_source}
\end{figure}
\input{table_eeg_runningtime_FFDIAG}




==> table_eeg_runningtime.tex <==

\begin{table}[!hbt!]
\begin{center}
\caption{Average running time in eye-blind signal separation}
\label{table:eeg_runningtime}
\begin{tabular}{||c | c | |}
\hline
Algorithm name & Avg running time(ms)\\
\hline
Pham & $\num{310.2600}$\\
\hline
RSDC & $\num{2.0568}$\\
\hline
RRSDC & $\num{6.6560}$\\
\hline
\end{tabular}
\end{center}
\end{table}

==> table_error_rumtime_rffdiag_ill_conditioned_backup.tex <==
\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for ill-conditioned matrices}
\label{table:ill_conditioned_rsdc}
\begin{tabular}{||c|c|c||}
    \hline
    Name & Time & Error \\
    \hline
    FFDIAG & $\num{6.41}$ & $\num{5.7e-14}$\\

    PHAM & $\num{884}$ & $\num{0.4}$\\
    
    QNDIAG & $\num{106}$ & $\num{4.7e-12}$\\
    
    RSDC & $\num{2.37}$ & $\num{3e-14}$\\
    
    RRSDC & $\num{2.91}$ & $\num{3.1e-14}$\\
    
    RFFDIAG & $\num{0.95}$ & $\num{1e-15}$\\
    
    \hline
    \end{tabular}
\end{center}
\end{table}


==> table_error_rumtime_rsdc_ill_conditioned.tex <==
\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for ill-conditioned matrices}
\label{table:ill_conditioned_rsdc}
\begin{tabular}{||c|c|c||}
    \hline
    Name & Time & Error \\
    \hline
    FFDIAG & $\num{683}$ & $\num{1.7e-07}$\\

    PHAM & $\num{866}$ & $\num{4.7e+07}$\\
    
    QNDIAG & $\num{423}$ & $\num{1.3e+07}$\\
    
    RSDC & $\num{3.25}$ & $\num{2.7e-06}$\\
    
    RRSDC & $\num{7.21}$ & $\num{2.8e-06}$\\
    
    \hline
    \end{tabular}
\end{center}
\end{table}


==> table_error_runtime_rffdiag_backup.tex <==

\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=10, n=10$}
\label{table:RSDC_10_10}
\begin{tabular}{||c|c|c|c|c|c|c||}
    \hline
    Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\   
    \hline
    FFDIAG & $\num{1.05}$ & $\num{1.1e-12}$ & $\num{1.04}$ & $\num{9e-07}$ & $\num{1.22}$ & $\num{9.22e-04}$\\

PHAM & $\num{31.6}$ & $\num{3.8e-13}$ & $\num{32.1}$ & $\num{1.2e-06}$ & $\num{32.8}$ & $\num{1.18e-03}$\\

QNDIAG & $\num{1.19}$ & $\num{8.3e-12}$ & $\num{1.15}$ & $\num{1.2e-06}$ & $\num{1.24}$ & $\num{1.18e-03}$\\

RSDC & $\num{0.28}$ & $\num{7.5e-15}$ & $\num{0.311}$ & $\num{3.9e-06}$ & $\num{0.31}$ & $\num{4.29e-03}$\\       

RRSDC & $\num{0.53}$ & $\num{8.4e-15}$ & $\num{1.77}$ & $\num{3.3e-06}$ & $\num{2.72}$ & $\num{2.55e-03}$\\       

RFFDIAG & $\num{0.246}$ & $\num{4.2e-16}$ & $\num{0.252}$ & $\num{9e-07}$ & $\num{0.389}$ & $\num{9.22e-04}$\\
    \hline
    \end{tabular}
\end{center}
\end{table}


\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=100, n=10$}
\label{table:RSDC_100_10}
\begin{tabular}{||c|c|c|c|c|c|c||}
    \hline
    Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\   
    \hline
    FFDIAG & $\num{6}$ & $\num{3.6e-13}$ & $\num{4.99}$ & $\num{1.1e-06}$ & $\num{7.12}$ & $\num{1.06e-03}$\\

PHAM & $\num{44.3}$ & $\num{2e-15}$ & $\num{53.7}$ & $\num{1.1e-06}$ & $\num{50.8}$ & $\num{1.08e-03}$\\

QNDIAG & $\num{17.1}$ & $\num{2.3e-15}$ & $\num{5.57}$ & $\num{1.1e-06}$ & $\num{4.31}$ & $\num{1.08e-03}$\\      

RSDC & $\num{0.461}$ & $\num{2.6e-14}$ & $\num{0.558}$ & $\num{4.8e-06}$ & $\num{0.509}$ & $\num{4.60e-03}$\\     

RRSDC & $\num{0.858}$ & $\num{2.4e-14}$ & $\num{10.3}$ & $\num{3.5e-06}$ & $\num{5.6}$ & $\num{3.38e-03}$\\       

RFFDIAG & $\num{0.573}$ & $\num{1.5e-15}$ & $\num{0.632}$ & $\num{1.1e-06}$ & $\num{1.51}$ & $\num{1.06e-03}$\\ 
    
    \hline
    \end{tabular}
\end{center}
\end{table}


\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=10, n=100$}
\label{table:RSDC_10_100}
\begin{tabular}{||c|c|c|c|c|c|c||}
    \hline
    Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\
    \hline
    FFDIAG & $\num{141}$ & $\num{1.8e-14}$ & $\num{147}$ & $\num{8.6e-07}$ & $\num{135}$ & $\num{7.71e-04}$\\
    
    PHAM & $\num{6.13e+03}$ & $\num{2.1e-15}$ & $\num{6.23e+03}$ & $\num{1.1e-06}$ & $\num{7.16e+03}$ & $\num{1.09e-03}$\\
    
    QNDIAG & $\num{119}$ & $\num{2.9e-15}$ & $\num{125}$ & $\num{1.1e-06}$ & $\num{374}$ & $\num{1.09e-03}$\\   
    
    RSDC & $\num{47}$ & $\num{1.2e-13}$ & $\num{48.7}$ & $\num{4.8e-05}$ & $\num{48.9}$ & $\num{7.76e-03}$\\    
    
    RRSDC & $\num{54.7}$ & $\num{1.4e-13}$ & $\num{78.1}$ & $\num{3.7e-05}$ & $\num{153}$ & $\num{4.36e-03}$\\  
    
    RFFDIAG & $\num{23.5}$ & $\num{1.4e-15}$ & $\num{27.8}$ & $\num{8.6e-07}$ & $\num{48}$ & $\num{1.37e-03}$\\ 
    
    \hline
    \end{tabular}
\end{center}
\end{table}

==> table_error_runtime_rsdc.tex <==

\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=10, n=10$}
\label{table:RSDC_10_10}
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\
\hline
JADE & $\num{29.2}$ & $\num{3.8}$ & $\num{33.7}$ & $\num{3.8}$ & $\num{34.8}$ & $\num{3.79e+00}$\\

FFDIAG & $\num{33.6}$ & $\num{2e-14}$ & $\num{34.1}$ & $\num{0.00013}$ & $\num{33.4}$ & $\num{1.93e-02}$\\

PHAM & $\num{33.5}$ & $\num{5.8e-14}$ & $\num{38.6}$ & $\num{0.00039}$ & $\num{40.3}$ & $\num{4.79e-02}$\\

QNDIAG & $\num{1.5}$ & $\num{3.6e-10}$ & $\num{1.45}$ & $\num{0.0039}$ & $\num{1.94}$ & $\num{3.36e-01}$\\

RSDC & $\num{0.35}$ & $\num{1.9e-14}$ & $\num{0.351}$ & $\num{5e-05}$ & $\num{0.364}$ & $\num{6.77e-03}$\\

RRSDC & $\num{0.626}$ & $\num{2e-14}$ & $\num{3.45}$ & $\num{3e-05}$ & $\num{3.49}$ & $\num{3.60e-03}$\\

ManNOJD & $\num{58.7}$ & $\num{0.052}$ & $\num{51.6}$ & $\num{0.052}$ & $\num{59.3}$ & $\num{5.13e-02}$\\

\hline
\end{tabular}
\end{center}
\end{table}


\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=10, n=100$}
\label{table:RSDC_10_100}
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\
\hline
JADE & $\num{6.38e+04}$ & $\num{16}$ & $\num{6.73e+04}$ & $\num{16}$ & $\num{6.36e+04}$ & $\num{1.58e+01}$\\

FFDIAG & $\num{5.8e+03}$ & $\num{4.7e-12}$ & $\num{6.09e+03}$ & $\num{0.0027}$ & $\num{5.99e+03}$ & $\num{2.00e-01}$\\

PHAM & $\num{6.87e+03}$ & $\num{3e-11}$ & $\num{7.13e+03}$ & $\num{0.025}$ & $\num{8.24e+03}$ & $\num{1.88e+00}$\\

QNDIAG & $\num{314}$ & $\num{4e-08}$ & $\num{321}$ & $\num{0.016}$ & $\num{396}$ & $\num{1.02e+00}$\\

RSDC & $\num{51.7}$ & $\num{1.2e-12}$ & $\num{50}$ & $\num{0.00063}$ & $\num{48.1}$ & $\num{2.36e-02}$\\

RRSDC & $\num{63}$ & $\num{1.4e-12}$ & $\num{131}$ & $\num{0.0005}$ & $\num{126}$ & $\num{1.41e-02}$\\

ManNOJD & $\num{2.05e+03}$ & $\num{0.071}$ & $\num{1.2e+03}$ & $\num{0.072}$ & $\num{1.32e+03}$ & $\num{7.10e-02}$\\

\hline
\end{tabular}
\end{center}
\end{table}


\begin{table}[!hbt!]
\begin{center}
\caption{Runtime and accuracy comparison for $d=30, n=30$}
\label{table:RSDC_30_30}
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
Name & Time $\epsilon_1$ & Error $\epsilon_1$ & Time $\epsilon_2$ & Error $\epsilon_2$ &Time $\epsilon_3$ &Error $\epsilon_3$\\
\hline
JADE & $\num{1.37e+03}$ & $\num{16}$ & $\num{1.32e+03}$ & $\num{16}$ & $\num{1.32e+03}$ & $\num{1.58e+01}$\\

FFDIAG & $\num{1.03e+03}$ & $\num{1.3e-11}$ & $\num{991}$ & $\num{0.00024}$ & $\num{984}$ & $\num{2.43e-02}$\\

PHAM & $\num{470}$ & $\num{5.9e-13}$ & $\num{445}$ & $\num{0.00063}$ & $\num{442}$ & $\num{6.48e-02}$\\

QNDIAG & $\num{6.82}$ & $\num{8.9e-09}$ & $\num{6.56}$ & $\num{0.0011}$ & $\num{6.81}$ & $\num{1.02e-01}$\\

RSDC & $\num{2.5}$ & $\num{3.8e-13}$ & $\num{2.49}$ & $\num{0.00017}$ & $\num{2.41}$ & $\num{1.35e-02}$\\

RRSDC & $\num{3.04}$ & $\num{3.9e-13}$ & $\num{13.5}$ & $\num{0.00011}$ & $\num{12.5}$ & $\num{9.71e-03}$\\

ManNOJD & $\num{179}$ & $\num{0.089}$ & $\num{179}$ & $\num{0.09}$ & $\num{178}$ & $\num{9.20e-02}$\\

\hline
\end{tabular}
\end{center}
\end{table}

==> table_image_separation_runningtime.tex <==
\begin{table}[!hbt!]
\begin{center}
\caption{Average running time in image separartion}
\label{table:image_separartion_runningtime}
\begin{tabular}{||c | c | |}
\hline
Algorithm name & Avg running time(ms)\\
\hline
RSDC & $\num{2.02}$\\
\hline
RRSDC & $\num{ 11.92}$\\
\hline
UWEDGE & $\num{40.01}$\\
\hline
FFDIAG & $\num{396.07}$\\
\hline
\end{tabular}
\end{center}
\end{table}
